Design optimisation of piezoelectric energy harvesters for bridge infrastructure

Vibrational energy harvested from the bridge excitation due to the traffic flow or the wind load can be supplied to sensors in a Structural Health Monitoring (SHM) system and help prolong its service life, reduce chemical battery waste and enable its use in remote locations. A common approach to designing a Piezoelectric Energy Harvester (PEH) consists in tuning its fundamental frequency to some target value (e.g., the fundamental frequency of a bridge). However, such approach does not answer the question if the chosen target frequency is optimal, and does not take into account the possibility to have multiple design configurations with the same fundamental frequency. In this work, we approach the problem of a PEH design optimisation in a rigorous way, using a PEH model based on the Kirchhoff-Love plate theory and Isogeometric Analysis (IGA), coupled with the Modal Order Reduction (MOR) approach and Runge-Kutta time integration method. The model is further equipped with the Particle Swarm Optimisation (PSO) algorithm that allows finding geometry which maximises energy output from a given base acceleration signal. A comprehensive study is conducted to infer the impact of a PEH geometry on its energy harvesting performance in a real-world setting by considering field health monitoring data of a large-scale cable-stayed bridge in NSW, Australia. A shape optimisation framework is developed based on acceleration events, i.e., where the level of response exceeds a certain threshold. Designs obtained in the event-based optimisation are then clustered to propose several best candidates for continuous energy generation. This work represents the first study on PEH design optimisation for real operational conditions.

==> Sections/section3.1.tex <==
\subsection{Excitations Required by the Optimisation}
\label{S:3.1}

Since, the vibration response of the bridge is continuously recorded, it is important to implement a further subsequent analysis in order to extract the events. Here, an event is defined by peaks of accelerations, such that accelerations greater than a certain threshold indicate the presence of an event. An event can be caused by environmental conditions such as wind excitation or by the passage of vehicles over the bridge, however in this framework, no distinctions are made regarding the cause. An example of a single event is presented in Figure \ref{event} where an acceleration threshold is set equal to 0.2 m/s$^2$. Here, the event time window is fixed to 30s and the location of the peak acceleration is forced to be at 10s. Note that all events will have the same time window and the same location for the peak acceleration. The events will be labelled with a number corresponding with the order of detection. 

==> Sections/section3.2.tex <==
\subsection{Proposed Framework for the Optimisation}
\label{S:3.2}

After the identification of the events, it is possible to apply the proposed optimisation procedure. The procedure consists of three parts: (1) the optimisation of the PEH for each event, (2) the clustering of optimal geometries, and (3) the estimation of the energy harvester for long time windows. The scheme of the procedure is shown in figure \ref{steps}, where the steps are detailed next.


In {\bf step 1}, shape optimisation is performed for each event (we call it Individual Event Optimisation) to identify the key excitation frequencies and limit the search space. Shape optimisation is performed for a representative number of events on the bridge (denoted by $N_e$). The optimisation for a single event is formalised as
\begin{equation}
    \label{optimal}
         \mathbf{x^*}= \text{arg}\,\max\limits_{\mathbf{x} \in \mathbf{X}} \, \vert E(\mathbf{x}\vert e) \vert 
\end{equation}

The objective function $E(\mathbf{x}\vert e)$ is the energy harvested from a specific event $e$ by a PEH whose geometry is defined by vector $\mathbf{x}$. The optimisation is established to obtain the geometrical parameters to maximise $E(\mathbf{x}\vert e)$. The optimal design is denoted by $\mathbf{x}^{\star}$. The optimal design for each event is schematically shown in Figure \ref{steps} assuming two design variables $\{$x$_1$, x$_2\}$. The objective function could be modified, for example to design PEHs considering the energy per unit of area. Particle Swarm Optimisation (PSO) \cite{poli2007particle,perez2007particle,kang2012damage} is the selected optimisation method due to its adequate performance for non-convex problems. PSO is an iterative method where a population of candidate solutions (or particles) moves in the search space towards the best solution. Each particle is associated with a position and a velocity, which are redefined in each iteration based on the individual and collective experience. The PSO method is expected to be an efficient optimisation algorithm because it is fast and computationally cheap; also it can be parallelised to further increase the computational efficiency.

\begin{figure}[h]
\centering\includegraphics[width=0.75\linewidth]{Figures/Steps3.pdf}
\caption{Overview of the proposed optimisation framework.}
\label{steps}
\end{figure}

%{\bf Step 2} consists in computing the energy harvested by each optimal device $\mathbf{x}^{\star}$, obtained in step 1, from all events, i.e.
%\begin{equation}
%    E(\mathbf{x^{\star}}) = \sum_{i = 1}^{N_e}E(\mathbf{x}^{\star}\vert e_i)
%    \label{sumE}
%\end{equation}

%The energy harvested is estimated using equation \ref{sumE} and the numerical integration of the power signal defined in the Eq. \ref{powersignal}. In Figure \ref{steps} (Step 2), optimal designs are shown together with the corresponding $E(\mathbf{x^{\star}})$, represented by circles of proportionally varying radii. The calculation of the energy harvested from the database of each optimal geometry allows for improving the clustering performance in the next stage.

{\bf Step 2} consists of the Clustering and Candidate Identification. The optimal geometries from each event tend to have a natural frequency close to one of the bridge's resonance frequencies. Thus, it is possible to group them in clusters based on the geometrical parameters (design variables). In Figure \ref{steps} (Step 2), optimal designs are schematically grouped into three clusters, denoted by yellow, red and green colours with their centroids denoted by black crosses. In this work, $k$-means \cite{kanungo2002efficient, diez2016clustering} is selected to cluster the geometries due to its ease of implementation, efficiency, empirical success, and adaptability in clusters of different shapes and sizes. $k$-means is an unsupervised machine learning algorithm that groups data (in that context, optimal designs) into one of $k$ clusters based on their characteristics (in that context, geometric parameters). The clusters are represented by a centroid which features are adjusted iteratively, minimising the distance with the assigned elements in the group. The number of clusters $k$ needs to be set before starting the algorithm, however, an arbitrary selection does not guarantee the best clustering result. To deal with this issue, the Silhouette Method \cite{yuan2019research} is also included in this framework to find the optimal $k$ value. The Silhouette method computes coefficients that measure how much a $point$ is similar to its cluster compared to others, providing a metric to evaluate how well each object has been classified. Finally, once the optimal designs have been grouped, the centroids calculated from the $k$-means are defined as candidates to be the optimal PEHs for continuous energy generation.

The last step, {\bf Step 3}, consists of assessing the Energy Harvested from a 24-hour acceleration signal (or any other time window) for each candidate obtained in Step 2. The purpose of this step is to select the best option (among the candidates) for continuous energy generation. In the real life scenario, this is the preferred design because the device should generate the optimal amount of energy independently on the traffic on the bridge. In Figure \ref{steps} (Step 3), energy generated by three candidates (centroids identified in Figure \ref{steps} (Step 2)) is shown schematically.      

The procedure proposed here, to optimise PEHs based on events (non-harmonic time series), is implemented later in the case study presented in Section 5 for an in service bridge. But first, and for the sake of comparison, Section 4 presents another case study where a PEH is optimised adopting a harmonic excitation.

%\sout{In Section \ref{....} 7?, the numerical simulation is performed for each candidate on a 24-hour acceleration signal to rank them in a continuous generation condition. The length of the time windows can vary according to the studied bridge's operation conditions. Now, when the traffic is relatively stable, a 24-hour signal of a labor day is a representative sample.}



==> Sections/section4.1.tex <==
\subsection{Damping Effect}
\label{S:4.1}
As it was mentioned in Section \ref{S:2}, proportional damping model is adopted in this study, thus, the damping matrix is defined as $\mathbf{C}=\alpha\mathbf{M} + \beta\mathbf{K}$ where the values of $\alpha$ and $\beta$ are considered invariant. The assumption of invariability of the constants has been used in previous works \cite{hurtado2022shape,junior2009electromechanical, peralta2020parametric}. If the problem is presented in modal coordinates, the damping matrix is redefined according to equation (\ref{mass_stiff_MOR}) as $\textbf{c}_o = \textbf{m}_o^{-1} \boldsymbol{\Phi}_o^T \textbf{C} \boldsymbol{\Phi}_o = \text{diag}(2\zeta_1\omega_1, … , 2\zeta_K\omega_K )$. In particular, the damping ratio is a good metric to describe the effect of changing shape. As the dominant vibration frequencies in bridges are low, it is common to design the PEH based on its first natural frequency. Hence, the most relevant damping ration of the PEH corresponds to $\zeta_1$.

Figure \ref{damping-Fig} shows the isocurves of the damping ratios $\zeta_1$ (black lines) in three design scenarios: Design 1 (left) in plane $(R, L)$, Design 2 (middle) in plane $(H, L)$ and Design 3 (right) in plane $(l, L)$. In all cases, the damping constants are $\alpha = 14.65$ rad/s and $\beta = 10^{−5}$ rad/s. In all three design scenarios, it is observed a strong dependence of $\zeta_1$ on $L$. Additionally, both $\zeta_1$ and the mass seem almost independent from the other parameter ($R$, $H$ or $l$).


%In case 1, the results are presented in $(R, L)$ plane. Here we observe that $\zeta$ increases with increasing length $L$ due to the increase of device's mass. However, the damping ratio stays constant with the variation of $R$ because this parameter does not affect the first vibration mode (as will be discussed in section \ref{sec:param_study} and seen from Figure \ref{Isocurve-Fig}, the change in $R$ does not affect the fundamental frequency $\omega_0$). In case 2, the isocurves are plotted in $(H, L)$ plane. Here, the effect of $L$ on $\zeta$ agrees with case 1. Meanwhile, $\zeta$ is almost independent of $H$ due to the pzt density and substructure density being similar between them, a change in $H$ does not mean a significantly mass variation. In case 3, damping ratios are shown in $(l, L)$ plane. The conclusion is similar to the previous cases. The damping ratio changes proportionally to $L$ and it is almost independent of $l$ due to the similar value of the pzt and substructure densities.}

\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/damping.pdf}
\caption{Isocurves for damping ratios $\zeta_1$ for the geometries in the three design scenarios: Design 1 (left), Design 2 (middle), Design 3 (right). The proportional damping coefficients correspond to $\alpha = 14.65$ rad/s and $\beta = 10^{-5}$ rad/s.}\label{damping-Fig}
\end{figure}



==> Sections/section4.2.tex <==
\subsection{Electrical Resistance Selection}
\label{S:4.2}
As it has been discussed in other works \cite{hurtado2022shape,junior2009electromechanical,erturk2008distributed, paquin2010improving}, the choice of external electrical resistance, $R_l$, directly affects the energy harvesting of a piezoelectric device. Therefore, energy generation can be significantly increased by choosing an optimal value of $R_l$. Then, the electrical resistance $R_l^*$ can be chosen to maximise the value of the power FRF at the first resonance frequency $\omega_o$. Note that $\omega_o$ is defined here as the frequency in which the power FRF has its maximum, thus, $\omega_o$ is expected to be close to the undamped frequency $\omega_1$. Such optimisation problem can be expressed as
\begin{equation}
    \label{OptimalRL}
         R_l^*= \text{arg}\,\max\limits_{R_l \in \mathbf{R}_l} \, \vert H_p(\omega_o, R_l\vert \mathbf{x}) \vert 
\end{equation}
with
\begin{equation}
    H_p(\cdot) = \frac{H_v(\cdot)^2}{R_l}
\end{equation} 
where $H_v(\cdot)$ is the voltage FRF defined in equation (\ref{Hv_equation}), and the vector $\mathbf{x}$ defines the device geometry ($\mathbf{x}=[L\,\,R]$ for Design 1, $\mathbf{x}=[L\,\,H]$ for Design 2, and $\mathbf{x}=[L\,\,l]$ for Design 3). Note that the power FRF is evaluated at the first resonance frequency $\omega_o$. However,  $\omega_o$  depends on the value of the external electrical resistance $R_l$, then $\omega_o$ can be considered as a function of $R_l$. Therefore, the value of $H_p(\omega_o(\Bar{R_l}), \Bar{R_l}\vert \mathbf{x})$ is calculated numerically and the optimisation problem, equation (\ref{OptimalRL}), is solved using the Nelder-Mead Simplex Method \cite{doi:10.1137/S1052623496303470}.

Figure \ref{load-Fig} shows the selected optimal values of the electrical resistance $R_l^*$ for the three studied designs. In general, the optimal resistance is almost independent of $L$ for values higher than 30 cm. For the other variables, there is a strong dependence on the optimal value $R_l^*$. The results show the importance of properly choosing the external resistance. The procedure to select the external electrical resistance will be used in the subsequent studies to increase power generation.
\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/load.pdf}
\caption{Isocurves for external optimal electrical resistances $R_l^*$ that maximise power generation at the fundamental frequency for the geometries in the three study cases: case 1 (left), case 2 (middle) and case 3 (right).}\label{load-Fig}
\end{figure}

 


==> Sections/section4.3.tex <==
\subsection{Optimization based on Harmonic Excitations}
\label{S:4.3}
A parametric study is carried out for the three design scenarios defined above. The electrical resistance adopted is optimal and selected following the procedure proposed in the previous section. The results are shown in Figure \ref{Isocurve-Fig}, where the effect of the size, shape and distribution of the piezoelectric material on the natural frequency $\omega_o$ and its respective power $H_o$ are studied. The isocurves for $\omega_o$ and $H_o$ in the ($R$, $L$) plane for Design 1 are represented in Figure \ref{Isocurve-Fig}a with a red and black line, respectively. As expected, $\omega_o$ decreases with increasing length $L$ due to the reduction in stiffness and the increase in mass. On the other hand, $\omega_o$ is almost independent of $R$. Concerning the maximum power $H_o$, the increase of $R$ and $L$ favours the generation of energy due to the increase in the device area and the amount of mass that increases the inertial effect. 

Figure \ref{Isocurve-Fig}b shows the $\omega_o$ (red line) and $H_o$ (black line) isocurves in the ($H$, $L$) plane for fully covered square devices (Design 2). Note that when the dimensionless thickness $H$ is increased for any $L$, a slight increase in the natural frequency $\omega_o$ is observed. It must be taken into account that the piezoelectric material has a lower density and Young's modulus than the substructure. This implies that the mass and stiffness of the device decrease when $H$ increases. However, the change in stiffness is the one that dominates the dynamic behaviour producing a decrement in $\omega_o$. Regarding the generated power $H_o$, it increases with $L$ mainly due to the increase in the PZT area. On the other hand, there is an increment and subsequently a reduction of $H_o$ with increasing $H$. This behaviour is the result of different factors. First, increasing the thickness of the piezoelectric layer decreases the inertial effect of the structure and consequently, there is less mechanical forcing over the PEH. Furthermore, the electromechanical coupling and the capacitance of the device are inversely proportional to the thickness $h_p$. In addition, a higher value of $H$ brings an increment in the flexibility of the device, which favours the increment in deformations during the excitation.

The isocurves of $\omega_o$ and $H_o$ in the ($l$, $L$) plane for Design 3 are shown in Figure \ref{Isocurve-Fig}c. As seen in the Figure, the natural frequency slightly increases when $l$ decreases. In this case, the increase in inertia in the area of the device's tip dominates the behaviour and produces the variation as mentioned earlier of $\omega_o$. On the other hand, similar to the previous cases, the natural frequency is proportional to $L$ despite increasing damping ratios. Regarding $H_o$, it increases and then decreases as $l$ decreases. It is due to the increase in the excitation force related to the greater inertia of the device. However, the decrease in $l$ implies a decrease in the area of the piezoelectric layers, responsible for the subsequent decrease in power $H_o$.

From these parametric studies it is possible to identify geometries that maximise the generated power $H_o$ for different natural frequencies $\omega_o$ (this is done by finding the intersection of the $\omega_o$-isoline with the $H_o$-isoline with highest value of $H_o$). These intersection points form lines, which are colored in grey and shown in Figure \ref{Isocurve-Fig}. Note that these results are independent of the bridge. Then, the designer can take the dominant vibration frequency of a particular bridge and select the geometry of the PEH based on the grey lines shown in Figure \ref{Isocurve-Fig}. 

\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/Isocurve.pdf}
\caption{Isocurves for peak amplitude $H_o$ of power FRF (black lines) and isocurves for natural frequencies $\omega_o$ (red lines) for the three design scenarios studied. The grey line corresponds to optimal geometries for any given natural frequency $\omega_o$.}\label{Isocurve-Fig}
\end{figure}

This parametric study reveals the importance of properly selecting the geometry of the PEH in order to maximise power output. However, the results presented in Figure \ref{Isocurve-Fig} are obtained adopting a single harmonic loading, i.e. $a_b = A_b e^{i\omega t}$. Hence, it is of interest to compare these results when a realistic excitation is applied over the PEH. This issue is addressed in the following section.

 





==> Sections/section4.tex <==
\section{Case Study 1: Optimization of PEHs for Bridges Assuming Harmonic Excitations}
\label{S:4}

In this section, a comprehensible study is carried out to understand how the piezoelectric device’s design impacts the energy harvesting in bridges. First, the effect of the damping on different geometries is discussed. Second, a procedure to select the electrical resistance is presented. Next, a parametric study is performed to infer the effect of the geometric parameters on the voltage generation considering harmonic accelerations. Finally, an optimisation problem to maximise the energy harvesting from a bridge is formulated and solved. The optimal results are compared with the parametric study. This case study serves as a benchmark problem to be compared with the procedure proposed in Section \ref{S:3}, this comparison is presented later in Section \ref{S:5}.

Five parameters define the geometry of the harvester: the total length $L$, the aspect ratio $R = W/L$ (relation between the width $W$ and the total length $L$), dimensionless piezoelectric length $l = L_{pzt}/L$ (relation between the length of the piezoelectric layers $L_{pzt}$ and the total length $L$), the total thickness $h = h_{s} + 2h_p$, and the dimensionless piezoelectric thickness $H = h_p/h$ (relation between the thickness of a piezoelectric layer $h_p$ and the total thickness $h$), please refers to Figure \ref{PEH-scheme} for reference. A bronze substructure and two PZT 5A piezoceramic sheets connected in series are considered. The corresponding material properties are given in Table \ref{mat_prop_demarqui22}.

Three design scenarios for parameters $(L, R, l, H)$ are carried out, all of them with $h = 1$mm. In each case, two parameters are fixed and two are considered as design variables: 
\begin{itemize}
    \item {\bf Design 1}: $H = 0.25$, $l = 1$, the design variables are: $L\in [10, 50]$ cm and $R\in [0.3, 1]$
    \item {\bf Design 2}: $R = 1$, $l = 1$, the design variables are: $L\in [10, 50]$ cm and $H\in [0.05, 0.45]$
    \item {\bf Design 3}: $R = 1$, $H = 0.25$, the design variables are: $L\in [10, 50]$ cm and $l\in [0.1, 1]$
\end{itemize}

The motivation to keep only two design variables instead of four is to help the visualisation and facilitate the interpretation of the results.

%In case 1, $L\in$[10, 50] cm and $R\in$[0.2, 1] are the decision variables. In case 2, $L\in$[10, 50] cm and $H\in$[0.1, 0.4] are the decision variables. Finally, $L\in$[10, 50] cm and $l\in$[0.1, 1] are the decision variable in case 3.\\


%\textcolor{red}{<--- parametric study is impossible to understand. Figures 6 and 7 are not explained, results presented in these figures are not analysed. What is being optimised under what conditions? Are we talking about harmonic input? Parameter $\zeta$ is not introduced, it is not clear how it's connected to constants $a$ and $b$. Please provide much clearer explanations with the precise formulation of the optimisation problem for $R_l$ and $\zeta$.}





 





==> Sections/section5.1.tex <==
\subsection{Optimisation based on Harmonic Excitation versus based on Time Series}
\label{S:5.1}

This section presents a comparison between the benchmark problem presented in case study 1 (optimization of PEHs based on harmonic excitations) and the optimal geometries identified by imposing excitations directly recorded from the bridge under study. For the sake of comparison, the design scenarios are the same of case study 1 but this time the optimisation is performed using 1000 events  following the procedure presented in Step 1 of the proposed framework (please refer to Section \ref{S:3.2}).


%where the vector $\mathbf{x} \in \mathbf{X}$ defines its geometry. The harvested energy is obtained from the numerical integration of the power signal $P(t)$ that derives from the proposed simulation method, where,
%\textcolor{blue}{
%\begin{equation}
%    \label{powersignal}
%    E(\mathbf{x}\vert e) = \int_{t_1}^{t_2}P(t, \mathbf{x}\vert e) dt = \int_{t_1}^{t_2}\frac{v^2(t, \mathbf{x}\vert e)}{R_l} dt
%\end{equation}
%}    

%A common option to implement in the Shape Optimization corresponds to the adoption of Heuristics-based techniques. 
%For the shape optimisation problem, we consider 1000 events occurring on the bridge and measured at sensor \textcolor{blue}{(14 located at the center of the bridge deck (see Figure 3).}

%In this work, Particle Swarm Optimisation (PSO) \cite{poli2007particle,perez2007particle,kang2012damage} is the selected as an optimisation method due to its adequate performance for non-convex problems. In simple words, PSO is an iterative method where a population of candidate solutions (or particles) moves in the search space towards the best solution. Each particle has associated a position and a velocity, which are redefined in each iteration based on the individual and collective experience.

The optimisation for each event is carried out based on the PSO method employing thirty particles. Figure \ref{ISOiterations} presents the iso-curves of the energy harvested from event 2 for the three design scenarios. In addition, the optimal geometries are marked with a star in the three figures. It is observed that the optimal geometry, obtained by the PSO, corresponds to the position estimated by the isocurves, which demonstrates the method converges to a correct value (global maximum). Convergence of the objective function is shown in Figure \ref{PSOiterations}. The figure shows that twenty iterations are enough to find the optimal value.
\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/Fig-isoPSO.pdf}
\caption{Isocurves for harvested energy from event 2 and the optimal geometry obtained from the PSO method: Design 1 (left), Design 2 (middle), Design 3 (right).}\label{ISOiterations}
\end{figure}

\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/Fig-iterPSO.pdf}
\caption{Optimal objective function in each iteration: Design 1 (left), Design 2 (middle), Design 3 (right).}\label{PSOiterations}
\end{figure}



%Three shape optimisation cases are carried out, which are based on the previous parametric studies. All cases started from a base configuration corresponding to a square profile (i.e. $H$=1), fully covered ($l$=1), with a total thickness equal to 1 [mm] and an $H$ of 0.25. In the case 1, $L$ and $R$ are the optimisation variables. Meanwhile, $L$ and $H$ are the optimisation variable in the case 2. Finally, $L$ and $l$ are the optimisation variable in the case 3. \textcolor{red}{(<-- I suggest to introduce the definition of case 1, case 2 and case earlier, in the parametric study, and describe them there clearly.)}

Figure \ref{ShapeOpt} shows the 1000 optimal PEH designs (one for each event) marked with blue, yellow and red dots for Designs 1, 2 and 3, respectively. Additionally, the figure shows the isocurve of the natural frequencies for different geometries (red line) and optimal designs using harmonic excitations  (grey area) identified in the benchmark problem (Case Study 1). The results show that for Design 1 and 2, the optimal geometries (blue and yellow dots) are aligned along the grey line, as expected. However, in Design 3, red dots show significant deviations from the grey line. These dispersions are explained by the discrepancies in predominant frequencies among the events as it is discussed next.

%\sout{However, dots tend to cluster around certain natural frequency values. Furthermore, the results for cases 1 and 2 are within the prediction area as expected while the results in case 3 present a greater dispersion than the predicted area, } This issue will be explored later.

\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/ShapeOpt.pdf}
\caption{Isocurves for fundamental frequencies $\omega_o$ (red lines). $(a)$ Optimal geometries for the 1000 Events in Design 1 (blue dots). $(b)$ Optimal geometries for the 1000 Events in Design 2 (yellow dots). $(c)$ Optimal geometries for the 1000 Events in Design 3 (red dots). The geometries related to events 2, 113, 304, 384, 781 and 718 are identified in three figures; also geometries for events 113 and 728 are denoted in the right figure. The geometries around the 2 Hz are marked by a rectangle in the left and central figures.}\label{ShapeOpt}
\end{figure}

To study the relationship between the dynamic characteristics of the device and the event frequency spectrum, Figure \ref{FRFevents} presents the comparison of FRFs of six optimal designs and the Fourier acceleration spectrum of their respective event for the three design scenarios. Six optimal designs are identified in Figure \ref{ShapeOpt} with the purpose to be compared, which correspond to events 2, 113, 304, 384, 781 and 718. First, note that the fundamental frequency of the piezoelectric devices is tuned with the predominant frequency of the acceleration spectrum. However, the acceleration peak is not always the one with the highest amplitude, such as the events 781 and 718 where the devices' fundamental frequency is tuned with the widest acceleration spectrum peak. Also, it is important to mention that there is consistency between the optimal FRFs for the three design scenarios, since the fundamental frequencies coincide in the six studied events. 
\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/FRFevents.pdf}
\caption{Comparison between the Fourier spectrum of the event acceleration signal and the FRFs of the optimal geometries obteined from the three design scenarios for events 2, 113, 304, 384, 781 and 718. }\label{FRFevents}
\end{figure}

Note that optimal designs within the grey line are those who generate the higher energy from their first vibration mode. This is valid for all PEHs in Designs 1 and 2. In this sense, there is consistency in these results, meaning that, by grouping the optimal designs around some key frequency, the corresponding events share same frequency characteristics. Figure \ref{FRFevents3} presents the Fourier spectra of the events associated with PEH design around the 2 Hz, which are identified by a rectangle in Figure \ref{ShapeOpt}-a and \ref{ShapeOpt}-b. As expected, it is seen that the predominated frequency is around 2 Hz, the same as the natural frequency of the optimal harvesters.

\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/SpectrumEvents.pdf}
\caption{Comparison of the normalised Fourier spectra of event acceleration signal around 2 Hz in Designs 1 and 2.}\label{FRFevents3}
\end{figure}

To understand the higher dispersion of the optimal geometries for Design 3, Figure \ref{FRFevents2} presents the comparison between the FRFs of three optimal designs and the Fourier acceleration spectrum of their respective event. The three optimal designs are identified in Figure \ref{ShapeOpt}-c, which correspond to events 2, 131 and 725. The three devices have the first natural frequency of 2 Hz. The high dispersion is explained by analysing the second natural frequency of the FRF. The main difference between Designs 1 and 2, against Design 3 is in the second natural frequency, which is more sensitive to change in parameter $l$ rather than parameters $R$ or $H$. The change in parameter $l$ allows increasing the energy generation from the second mode of vibration, slightly decreasing the energy generation from the first one, leading to a higher energy overall. Therefore, the main conclusion from this study is that according to the spectral characteristics of an event, in some cases it is better to use devices that harvest energy only around the first natural frequency, while in others it is more efficient to harvest energy simultaneously from the first two natural frequencies. Despite the fact that it might reduce the energy generation in the first range in order to favour energy generation in the second. 
\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/FRF3dots.pdf}
\caption{Comparison between the Fourier spectrum of event acceleration signal and the FRFs of the optimal geometries from the three shape optimisation cases for events 2, 131 and 725.}\label{FRFevents2}
\end{figure}

The results of this section can be summarised as follows. The optimisation problem using the event acceleration response in the bridge yields the results, expected from the FRF analysis and parametric studies. Obtained results are consistent among the studied cases. It was found that not always the best option is to tune and maximise the energy generation in one frequency (prediction areas). Also, the natural frequency of the optimal device is not always close to the highest peak of the acceleration spectrum of the corresponding event. All these issues are considered by the direct optimisation of the events in the time domain, giving it greater robustness than the design obtained by simply tuning the natural frequency of the device with a target value. Nevertheless, the optimal designs from different events present a high dispersion in case 3, where one of the design parameters is the ratio between the PZT-layer length and the overall device length, which makes the design sensitive with respect to the second fundamental frequency. In practice, we are interested in designing one or a limited number of piezoelectric devices for a continuous generation; thus, it is not feasible to design a device for each event or perform an optimisation process in long time windows due to computational limitations. In that sense, the next section will present an optimisation framework for designing piezoelectric devices for a continuous generation based on the results presented in this section.

%\textcolor{red}{I also don't understand the transition from section 5 to section 6. We claim that our FRF approach works perfectly fine for case 1 and case 2 and the results are already consistent across all events, then why do we need a further study and further optimisation for large number of events? I am asking only about case 1 and case 2. }

%This is a problem because the main idea of this procedure is to choose a limited number of PEH's geometry to maximise the continuous generation, but increasing the number of Events increases the number of candidates. Some solutions could be to perform the optimisation process considering all the event data or long time windows. However, it is not feasible due to the extensive computational resources requirements. Therefore, in the next section we present an optimisation Framework to deal with the mentioned problem and obtain a reduced number of candidates to maximise the continuous generation.






==> Sections/section5.2.tex <==




\subsection{Optimisation based on Time Series for a Time Window of 24hrs}
\label{S:5.2}


The optimisation framework proposed in Section \ref{S:3} is applied to the cable-stayed bridge presented here. The framework is expected to offer candidates to maximise the energy harvested in continuous operation. 1000 Events are considered in this case as a representative number for this bridge because it is the approximate number of events that occur during a week even though the selected events are drawn from different periods. The PEH materials are chosen the same as in Section \ref{S:4}. A serial connection between the piezoelectric layers is considered, and the selected electrical resistance for each geometry is the one that maximises the peak of the FRF at the fundamental frequency. Five design parameters describe the geometry: total length $L\in$[10, 50] cm, aspect ratio $R\in$[0.3, 1], dimensionless piezoelectric length $l\in$[0.1, 1], dimensionless piezoelectric thickness $H\in$[0.05, 0.45], and total thickness $h$ which is assumed constant and equal to 1 mm. Design variables are defined as
\begin{equation}
    \mathbf{x} = \{R, L, l, H\}
\end{equation}

First, the individual event optimisation was performed for 1000 events. As a result, 1000 optimal geometries were obtained. It was observed that all optimal geometries correspond to $R = 1$, which is in agreement with the results in Section \ref{S:4.3}, hence variable $R$ is omitted from the further analysis. Optimal designs are shown in Figure \ref{OptimalGeometriesCS1} in $L-l-H$ space and their projections in the $L-l$ and $L-H$ planes. From Figure \ref{OptimalGeometriesCS1}b it can be seen that the results present a high dispersion in the variable $L$ and low in the variable $H$. The high dispersion in $L$ is explained by its strong dependence with the natural frequency of the device, the high variability in the predominant frequencies between the events, and the fact that the devices tend to synchronize to the event´s predominant frequencies. In Figure \ref{OptimalGeometriesCS1}c, it is possible to observed a dispersion in the variable $l$. This is explained by the fact that the devices tune their first two resonance frequencies with some bridge's natural frequencies in some events. In particular, $l$ allows increasing the energy generation from the second mode of vibration, slightly decreasing the energy generation from the first one, leading to an overall higher harvested energy according to the specific spectral characteristic of the event.

\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/Fig14.pdf}
\caption{Optimal geometries for 1000 Events in the $L−l−H$ space (left), $L−H$ plane (middle) and $L−l$ plane (right).}
\label{OptimalGeometriesCS1}
\end{figure}

%After the individual event optimisation, the amount of energy that each optimal design harvests from all events is quantified, which will be used to improve the clustering performance in the next step. Figure \ref{EnergyEventsCS1} shows the results, where the size of the indicator points of each optimal geometry is proportional to the energy harvested from all events. The results are presented in the $L-l-H$ space and their projection in the $L-l$ and $L-H$ planes. From Figure \ref{EnergyEventsCS1} one can notice that the most significant amount of energy is generated by devices with a length $L$ around 45 cm, whose fundamental frequency is close to 2 Hz. This gives us a first estimate of the best candidates for the energy generation from a continuous 24 hour signal. However, this analysis does not consider the occurrence of similar events between them.

%\begin{figure}[h]
%\centering\includegraphics[width=1.0\linewidth]{Figures/FigDotsEnergy.pdf}
%\caption{Energy harvested by the 1000 optimal devices from the full event database in the $L−l−H$ space (left), $L−H$ plane (middle) and $L−l$ plane (right).}
%\label{EnergyEventsCS1}
%\end{figure}

After the individual event optimisation, cluster identification is carried out where the optimal geometries are grouped based on the similarity between them, taking into account the geometric variables $L$, $l$ and $H$. The cluster number is determined based on the Silhouette coefficient, which allows evaluating how well each geometry has been classified in their cluster with respect to the others. The results for different cluster numbers are presented in Figure \ref{SilhouetteCS1}, where it is concluded that the optimal number is 6 clusters. Next, cluster identification is performed based on the $k$-means algorithm. The six clusters and their respective centroids are presented in Figure \ref{clusterCS1}. In this framework, the centroids are considered to be representative candidates of each cluster. Finally, the 1000 optimal geometries have been reduced to six candidates that will be evaluated for the continuous power generation.

\begin{figure}[h]
\centering\includegraphics[width=0.5\linewidth]{Figures/Fig16.pdf}
\caption{Silhouette Coefficient for different $k$-values applied to the 1000 optimal geometries.}
\label{SilhouetteCS1}
\end{figure}

\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/Fig17.pdf}
\caption{Six clusters of the optimal geometries for 1000 events in the $L−l−H$ space (left), $L−H$ plane (middle) and $L−l$ plane (right). Black crosses denote candidates (centroid of each cluster).}
\label{clusterCS1}
\end{figure}

The cable stayed bridge studied in this work is generally not subjected to high traffic, so the frequency of occurrence of events is low. Therefore, the optimisation framework is also evaluated in time windows without events (i.e., small oscillations in response to environmental conditions) since this condition prevails over time. In addition, this analysis will function as a control group for the present case study. 100 time windows of 30 seconds without events are extracted from the same period considered in the 1000 event extraction. Then for each time window, the corresponding acceleration signal is used as an input in the optimisation problem. The results of such individual optimisation are shown in Figure \ref{noEventCS1}. Note that the optimal geometries present a low dispersion, as expected, since the oscillations in the absence of traffic are consistent in time. Therefore, it seems reasonable to consider only one design candidate to evaluate it in the continuous operation and compare it with the other six candidates defined above.

\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/Fig18.pdf}
\caption{Optimal geometries for 100 time windows of 30 seconds without events in the $L−l−H$ space (left), $L−H$ plane (middle) and $L−l$ plane (right).}
\label{noEventCS1}
\end{figure}

Finally, the seven PEH candidates are evaluated under 24 hour continuous operation conditions. Figure \ref{FRFcanditates} presents their power FRFs, where it is possible to identify their natural frequencies. Note that these values coincide with the frequencies, where the optimal geometries from the optimisation in Section \ref{S:5.1} are grouped. It is also important to note that the first two natural frequencies of candidates 1 and 2 coincide and only vary in their amplitude in the FRF, which agrees with the results observed and discussed previously in Design 3 of Section \ref{S:5.1}. Next, Figure \ref{energy24hrs} presents the energy harvested from a 24 hour signal by the seven candidates. We can conclude that the candidates with the highest performance are the candidates whose first natural frequency is around 2 Hz, with candidate 7 being the one that generates the most energy. Note that candidate 7 is representative of event-less window optimisations. However, the energy harvested by the best candidate is only 0.47\% and 3.79\% higher than candidates 1 and 2, respectively. 

\begin{figure}[h!]
\centering\includegraphics[width=1.0\linewidth]{Figures/frfCandidates.pdf}
\caption{Power FRF of the seven candidates to assess energy harvested from a continuous 24-hour signal.}
\label{FRFcanditates}
\end{figure}

\begin{figure}[h]
\centering\includegraphics[width=0.75\linewidth]{Figures/Fig19.pdf}
\caption{Energy harvested from a 24 hour signal by the seven candidates.}
\label{energy24hrs}
\end{figure}

Although, the optimisation framework suggests that the optimal device is the one obtained from the optimisation of the windows without events, this cannot be generalised to any bridge since it depends on different factors such as the structure of the bridge, the vehicular characteristics and the frequency of the traffic, all of them impacting the event's occurrence rate. The factors mentioned are intrinsically included in the framework and are the ones that define dissimilar results for each context. In order to highlight the impact of the occurrence rate, it is decided to include Table \ref{CandidatevsCluster}. This table contains the expected energy harvested (in a time frame of 30s) by each candidate when they are excited with events of different clusters. For example, if candidate 1 is excited with an event belonging to cluster 2, then it is expected to produce 6.10$\mu$J in 30s. As it is expected, the higher energy for an event is produced by its correlative candidate, e.g., for an event of cluster 2, the best candidate is also the number 2. Also, it is important to note that the highest energy is harvested when candidate 6 is excited with an event belonging to cluster 6. However, candidate 6 in Figure \ref{energy24hrs} is the candidate that generates the lowest amount of energy accumulated in 24 hours. Contrary, it is possible to observe that the lowest amount of energy generated by any candidate occurs when no events are presented in the excitation (column 7 in Table \ref{CandidatevsCluster}). However, the candidate 7 is the one that generates the most amount of accumulated energy in 24hrs. This situation is explained by the occurrence rate of an event belonging to a specific cluster. The last row of the table incorporates the mentioned occurrence rate. Here, it is observed that events of cluster 6 have an occurrence rate close to 0.5\%, while the occurrence rate for an event-less excitation is close to 95\%. As it is seen, the occurrence rate plays a determinant role in the optimisation. Furthermore, the information in this table could be used to estimate the energy produced by any candidate in any time frame. For example taking candidate 1, if the first row (corresponding to candidate 1) is weighted by the occurrence rate (last row) and the result is summed, then the expected energy harvested by candidate 1 in 30s is obtained. Then, the result could be linearly scaled to estimate the expected energy harvested in a different time frame.

Table \ref{harvestedEnergyComparation} compares the energy generated in this work with some previous studies. Although the results coincide with the order of magnitude, it does not exceed the harvested energy from other studies. This is mainly due to the characteristics and ways the bridge-vehicle system is modeled in these works. In particular, the fact that in \cite{zhang2018experimental} the research was carried out in an experimental setup with a scaled bridge-vehicle system, allows the generation of energy to occur in higher frequencies, which benefits the efficiency of the devices. On the other hand, In \cite{romero2021energy}, the data used corresponds to a railway bridge, where are higher available mechanical energy compared to vehicular bridges for the greater mass and speed of trains. The same happens in \cite{song2019finite}, where the numerical simulation is modeled on a bridge-train system.

\begin{table}[h!]
\centering
\caption{Comparison of the harvested energy from the present work compared to some previous studies.}
\renewcommand{\arraystretch}{1.25}
\label{harvestedEnergyComparation}
\begin{tabular}{lrll}
\hline
This Work     & $\sim$0-7.8  & $\mu$J & for each passing vehicle \\
              & 2.5          & mJ     & in 24 hours              \\
Romero et. al \cite{romero2021energy} & 3.6          & mJ     & for each passing train   \\
              & $\sim$0-0.84 & mJ     & in 3.5 hours             \\
Song \cite{song2019finite}         & $\sim$0-462  & mJ     & for each passing train \\
Zhang et. al \cite{zhang2018experimental}   & 60-565       & $\mu$J & for each passing vehicle \\ \hline
\end{tabular}
\end{table}

Another aspect which was not considered in this work is dependence of the optimisation results on the device's position on the bridge. In general, the device's position is associated with the different vibration modes of the bridge, so the amplitude associated with specific vibration frequencies is affected. In particular, the position selected in this case study favours the first mode of vibration and explains why a more significant number of optimal devices from the individual optimisation will cluster around 2 Hz. However, it is not necessarily the optimal position on the bridge and other positions should be studied.

%\textcolor{red}{I have yet to add a comparative table with previous studies.}
%\textcolor{red}{Not sure if it's possible, but I'll ask anyway :) Can we add a table comparing energies generated from other studies (I think you had a table in your slides for HDR review. With the energy that we obtained. Is it possible to compare?)}


%\begin{figure}[h]
%\centering\includegraphics[width=1.0\linewidth]{Fig1Area.pdf}
%\caption{caption}
%\label{steps}
%\end{figure}


\begin{table}[h!]
\centering
\caption{Expected energy harvested (in a time frame of 30s) by all candidates when they are excited with events belonging to different clusters. The energy is in $\mu$J. The last row corresponds to the occurrence rate of an event belonging to a particular cluster for the case study}
\renewcommand{\arraystretch}{1.25}
\label{CandidatevsCluster}
\begin{tabular}{cllllllll}
\cline{3-9}
\multicolumn{1}{l}{}                            &                        & \multicolumn{7}{c}{Event's Cluster}                                                                                                                                           \\ \cline{3-9} 
\multicolumn{1}{l}{}                            &                        & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{6} & \multicolumn{1}{c}{7} \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{\rotatebox{90}{Candidate}	}} & \multicolumn{1}{l|}{1} & 5.50                   & 6.10                   & 2.13                   & 1.40                   & 1.06                   & 5.43                   & 0.54                   \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{l|}{2} & 5.31                   & 6.26                   & 2.00                   & 1.37                   & 1.15                   & 6.28                   & 0.52                   \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{l|}{3} & 3.30                   & 3.84                   & 2.92                  & 1.68                   & 1.30                    & 3.56                  & 0.22                   \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{l|}{4} & 1.36                   & 1.61                   & 1.54                   & 1.89                   & 0.88                   & 1.87                   & 0.03                   \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{l|}{5} & 1.86                   & 2.29                   & 2.11                   & 1.74                   & 1.43                   & 2.56                   & 0.07                   \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{l|}{6} & 0.91                   & 3.66                   & 0.60                   & 0.76                   & 0.98                   & 7.76                   & 0.00                   \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{l|}{7} & 5.51                   & 6.05                   & 2.00                   & 1.34                   & 1.03                   & 5.42                   & 0.55                  \\ \hline
                  Occurrence rate        &  & 0.017                  & 0.006                  & 0.018                  & 0.003                  & 0.001                  & 0.005                  & 0.950\\
                           \hline
\end{tabular}
\end{table}



==> Sections/section5.tex <==
\section{Case Study 2: Optimization of PEHs for an in Service Bridge Using Time Series Excitations} 
\label{S:5}
A cable-stayed bridge, shown in  Figure~\ref{fig:fig1},  carrying one traffic lane and one pedestrian lane with a maximum loading capacity of 30 tons over the Great Western Highway in the state of New South Wales (NSW), Australia, was analysed in \cite{alamdari2019multi}, and it is chosen as a case study in this work. The structural system consists of a composite steel-concrete deck spanning over 46.2m and an A-shaped steel pylon with a height of 33m. The width and the depth of the concrete deck are uniform at 6.30m and 0.16m, respectively. The deck is supported by four longitudinal girders which are internally attached by a set of seven cross girders (CGs), see Figure \ref{fig:sensor}. Sixteen semi-fan arranged pre-tensioned stayed-cables with a diameter of 38mm are anchored on steel tower and cross girders. 

A dense array of timely-synchronised sensors, including strain gauges and accelerometers have been installed on the bridge since 2016 \cite{alamdari2019damage}. Twenty-four uni-axial accelerometer sensors were permanently placed under the deck at the intersection of the girders and floor beams to measure the vertical acceleration of the bridge, see Figure \ref{fig:sensor}. These sensors are low-noise capacitive accelerometers [2210-002 Silicon Design] which can detect acceleration within the range of $\pm 2g$ with a sensitivity of 2,000 mV/g.The signal conditioning and data logging software consist of an embedded PC and HBM Quantum-X data logger to record data. This system provides an integrated and reliable device to log high-quality data with 24-bit resolution with bandwidth capability of 0–3 kHz. All data are collected at a default sample rate of 600 Hz with an anti-aliasing filter. The 3-dB cutoff frequency of the filter is 100 Hz and it is a fourth-order Bessel low-pass filter. \begin{figure}[h]
	\centering
	\includegraphics[width=0.6\textwidth]{Figures/1.jpg}
			\caption{Illustration of the cable-stayed bridge located in the state of NSW, Australia.}
			  \label{fig:fig1}
\end{figure}

\begin{figure}[h]
	\centering\includegraphics[width=1.0\linewidth]{Figures/accelerationArray2.pdf}
			\caption{Illustration of the sensor layout under the deck.}
			  \label{fig:sensor}
\end{figure}

Following the procedure proposed in Section \ref{S:3.1}. 1000 events were extracted in a period of seven days and were numerically labeled in order of appearance. The acceleration threshold to define the event was set in 0.15 m/s$^2$. The events can be caused by environmental conditions or by the passage of vehicles over the bridge. Acceleration measured at sensor A14 was chosen for this study due to its location at the center of the bridge. Based on the conclusions of some previous studies \cite{zhang2018experimental,romero2021energy}, the PEH performance for such location is expected to be higher. The event labeled as 2 was already presented in Figure \ref{event}. All events are confined by a time window of 30s where its peak acceleration occurs at the time of 10s.

Although the bridge has only one traffic line, the vehicles can travel in both directions because the traffic flow is not high. Also, the first natural natural frequencies are low, i.e., 2 and 3.5 Hz for the first two modes, respectively \cite{alamdari2019damage}. 

%\textcolor{red}{I have to add bridge's features}
%\textcolor{red}{Can we collect here in bullet points the main features of this bridge most relevant to this work. 1. fundamental frequency of 2 Hz, 2. Low traffic, 3. why we chose location A14, etc..... what else?}



==> Sections/sectionX.1.1.tex <==
\subsubsection{Electrical Resistance Selection}

Energy generation can be significantly increased by choosing an optimal value of $R_l$. Then, the electrical resistance $R_l^*$ can be chosen to maximise the value of the power FRF at the first resonance frequency $\omega_o$. Note that $\omega_o$ is defined here as the frequency in which the power FRF has its maximum, thus, $\omega_o$ is expected to be close to the undamped frequency $\omega_1$. Such optimisation problem can be expressed as
\begin{equation}
    \label{OptimalRL}
         R_l^*= \text{arg}\,\max\limits_{R_l \in \mathbf{R}_l} \, \vert H_p(\omega_o, R_l\vert \mathbf{x}) \vert 
\end{equation}
with
\begin{equation}
    H_p(\cdot) = \frac{H_v(\cdot)^2}{R_l}
\end{equation} 
where $H_v(\cdot)$ is the voltage FRF defined in equation (\ref{Hv_equation}), and the vector $\mathbf{x}$ defines the device geometry ($\mathbf{x}=[L\,\,R]$ for Design 1, $\mathbf{x}=[L\,\,H]$ for Design 2, and $\mathbf{x}=[L\,\,l]$ for Design 3). Note that the power FRF is evaluated at the first resonance frequency $\omega_o$. However, $\omega_o$  depends on the value of the external electrical resistance $R_l$, then $\omega_o$ can be considered as a function of $R_l$. Therefore, the value of $H_p(\omega_o(\Bar{R_l}), \Bar{R_l}\vert \mathbf{x})$ is calculated numerically and the optimisation problem, equation (\ref{OptimalRL}), is solved using the Nelder-Mead Simplex Method \cite{doi:10.1137/S1052623496303470}.

Figure \ref{load-Fig} shows the selected optimal values of the electrical resistance $R_l^*$ for the three studied designs. In general, the optimal resistance is almost independent of $L$ for values higher than 30 cm. For the other variables, there is a strong dependence on the optimal value $R_l^*$. The results show the importance of properly choosing the external resistance. The procedure to select the external electrical resistance will be used in the subsequent studies to increase power generation.
\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/load.pdf}
\caption{Isocurves for external optimal electrical resistances $R_l^*$ that maximise power generation at the fundamental frequency for the geometries in the three study cases: Design 1 (left), Design 2 (middle) and Design 3 (right).}\label{load-Fig}
\end{figure}


==> Sections/sectionX.1.2.tex <==
\subsubsection{Optimisation and Parametric Study}

A parametric study is carried out for the three design scenarios defined above. The electrical resistance adopted is optimal and selected following the procedure proposed in the previous section. The results are shown in Figure \ref{Isocurve-Fig}, where the effect of the size, shape and distribution of the piezoelectric material on the natural frequency $\omega_o$ and its respective power $H_o$ are studied. The isocurves for $\omega_o$ and $H_o$ in the ($R$, $L$) plane for Design 1 are represented in Figure \ref{Isocurve-Fig}a with a red and black line, respectively. As expected, $\omega_o$ decreases with increasing length $L$ due to the reduction in stiffness and the increase in mass. On the other hand, $\omega_o$ is almost independent of $R$. Concerning the maximum power $H_o$, the increase of $R$ and $L$ favours the generation of energy due to the increase in the device area and the amount of mass that increases the inertial effect.

Figure \ref{Isocurve-Fig}b shows the $\omega_o$ (red line) and $H_o$ (black line) isocurves in the ($H$, $L$) plane for fully covered square devices (Design 2). Note that when the dimensionless thickness $H$ is increased for any $L$, a slight increase in the natural frequency $\omega_o$ is observed. It must be taken into account that the piezoelectric material has a lower density and Young's modulus than the substructure. This implies that the mass and stiffness of the device decrease when $H$ increases. However, the change in stiffness is the one that dominates the dynamic behaviour producing a decrement in $\omega_o$. Regarding the generated power $H_o$, it increases with $L$ mainly due to the increase in the PZT area. On the other hand, there is an increment and subsequently a reduction of $H_o$ with increasing $H$. This behaviour is the result of different factors. First, increasing the thickness of the piezoelectric layer decreases the inertial effect of the structure and consequently, there is less mechanical forcing over the PEH. Furthermore, the electromechanical coupling and the capacitance of the device are inversely proportional to the thickness $h_p$. In addition, a higher value of $H$ brings an increment in the flexibility of the device, which favours the increment in deformations during the excitation.

The isocurves of $\omega_o$ and $H_o$ in the ($l$, $L$) plane for Design 3 are shown in Figure \ref{Isocurve-Fig}c. As seen in the Figure, the natural frequency $\omega_o$ slightly increases when $l$ decreases because the increase in inertia in the area of the device's tip. On the other hand, similar to the previous cases, the natural frequency is proportional to $L$ despite increasing damping ratios. Regarding $H_o$, it increases and then decreases as $l$ decreases. It is due to the increase in the excitation force related to the greater inertia of the device. However, the decrease in $l$ implies a decrease in the area of the piezoelectric layers, responsible for the subsequent decrease in power $H_o$.

From these parametric studies, it is possible to identify geometries that maximise the generated power $H_o$ for different natural frequencies $\omega_o$ (this is done by finding the intersection of the $\omega_o$-isoline with the $H_o$-isoline with highest value of $H_o$). These intersection points form lines, which are coloured in grey and shown in Figure \ref{Isocurve-Fig}. Note that these results are independent of the bridge. Then, the designer can take the dominant vibration frequency of a particular bridge and select the geometry of the PEH based on the grey lines shown in Figure \ref{Isocurve-Fig}. 

\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/Isocurve.pdf}
\caption{Isocurves for peak amplitude $H_o$ of power FRF (black lines) and isocurves for natural frequencies $\omega_o$ (red lines) for the three design scenarios studied. The grey lines correspond to optimal geometries for any given natural frequency $\omega_o$.}\label{Isocurve-Fig}
\end{figure}

This parametric study reveals the importance of properly selecting the geometry of the PEH in order to maximise power output. However, the results presented in Figure \ref{Isocurve-Fig} are obtained adopting a single harmonic loading, i.e. $a_b = A_b e^{i\omega t}$. Hence, it is of interest to compare these results when a realistic excitation is applied over the PEH. This issue is addressed in the following section.


==> Sections/sectionX.1.tex <==
\subsection{Parametric Study and Optimisation assuming Harmonic Excitation}\label{design_cases}

In this section, a parametric study is performed to infer how the piezoelectric device’s design impacts the energy harvesting assuming harmonic excitations. Next, the optimal value for the different excitation frequencies is identified and will be the benchmark for the optimisation based on the bridge time series. Three design scenarios for parameters $(L, R, l, H)$ are carried out, all of them with $h = 1$mm. In each case, two parameters are fixed and two are considered as design variables: 
\begin{itemize}
    \item {\bf Design 1}: $H = 0.25$, $l = 1$, the design variables are: $L\in [10, 50]$ cm and $R\in [0.3, 1]$
    \item {\bf Design 2}: $R = 1$, $l = 1$, the design variables are: $L\in [10, 50]$ cm and $H\in [0.05, 0.45]$
    \item {\bf Design 3}: $R = 1$, $H = 0.25$, the design variables are: $L\in [10, 50]$ cm and $l\in [0.1, 1]$
\end{itemize}
The motivation to keep only two design variables instead of four is to help the visualisation and facilitate the interpretation of the results.
As it has been discussed in other works \cite{hurtado2022shape,junior2009electromechanical,erturk2008distributed, paquin2010improving}, the choice of external electrical resistance, $R_l$, directly affects the energy harvesting of a specific piezoelectric geometry. Therefore, energy generation can be significantly increased by choosing an optimal value of $R_l$. In this way, a procedure to select the electrical resistance for each geometry is presented next. The procedure is then used in the parametric study and the subsequent optimisation processes in order to have consistency between the results.


==> Sections/sectionX.2.tex <==
\subsection{Optimisation based on Time-Series versus Harmonic Excitation}
\label{s:X.2}

This section presents a comparison between the benchmark problem presented in previous section (optimisation of PEHs based on harmonic excitations) and the optimal geometries identified by imposing excitations directly recorded from the bridge under study. For the sake of comparison, we use the same three design scenarios, as described in Section \ref{design_cases}, but this time the optimisation is performed using 1000 events following the procedure presented in Step 1 of the proposed framework in Section \ref{S:3}.

A dense array of timely-synchronised accelerometers have been installed on the bridge since 2016 \cite{alamdari2019damage}. Twenty-four uni-axial accelerometer sensors were permanently placed under the deck at the intersection of the girders and floor beams to measure the vertical acceleration of the bridge, see Figure \ref{fig:sensor}. These sensors are low-noise capacitive accelerometers [2210-002 Silicon Design] which can detect acceleration within the range of $\pm 2g$ with a sensitivity of 2,000 mV/g. The signal conditioning and data logging software consist of an embedded PC and HBM Quantum-X data logger to record data. This system provides an integrated and reliable device to log high-quality data with 24-bit resolution with a bandwidth capability of 0–3 kHz. All data are collected at a default sample rate of 600 Hz with an anti-aliasing filter. The 3-dB cut-off frequency of the filter is 100 Hz and it is a fourth-order Bessel low-pass filter.
\begin{figure}[h]
	\centering\includegraphics[width=1.0\linewidth]{Figures/accelerationArray2.pdf}
	\caption{Illustration of the sensor layout under the deck. Acceleration response at sensor A14 was chosen for the study.}
	 \label{fig:sensor}
\end{figure}
Here, an event is defined by peaks of accelerations, such that accelerations greater than a certain threshold indicate the presence of an event. An event can be caused by environmental conditions such as wind excitation or by the passage of vehicles over the bridge, however in this framework, no distinctions are made regarding the cause. The acceleration threshold to define the event was set at 0.15 m/s$^2$. The event time window is fixed to 30s and the location of the peak acceleration is forced to be at 10s. Note that all events will have the same time window and the same location for the peak acceleration. 1000 events were extracted in a period of seven days and were labelled in order of appearance. An example of a single event (event 2) is presented in Figure \ref{event02}a. The acceleration measured at sensor A14 was chosen for this study due to its location at the center of the bridge. Based on the conclusions of some previous studies \cite{zhang2018experimental,romero2021energy}, the PEH performance for such a location is expected to be higher. 

%1000 events were extracted in a period of seven days and were numerically labelled in order of appearance. The acceleration measured at sensor A14 was chosen for this study due to its location at the center of the bridge. Based on the conclusions of some previous studies \cite{zhang2018experimental,romero2021energy}, the PEH performance for such a location is expected to be higher. 
%The event labelled as 2 was already presented in Figure \ref{event02}a. All events are confined by a time window of 30s where its peak acceleration occurs at the time of 10s.

The optimisation for each event is carried out based on the PSO method employing thirty particles. Figure \ref{ISOiterations} presents the iso-curves of the energy harvested from event 2 for the three design scenarios. In addition, the optimal geometries are marked with a star in the three figures. It is observed that the optimal geometry, obtained by the PSO, corresponds to the position estimated by the isocurves, which demonstrates that the method converges to a correct value (global maximum). Convergence of the objective function is shown in Figure \ref{PSOiterations}. The figure shows that twenty iterations are enough to find the optimal value.
\begin{figure}[h!]
\centering\includegraphics[width=1.0\linewidth]{Figures/Fig-isoPSO.pdf}
\caption{Isocurves for harvested energy from event 2 and the optimal geometry obtained from the PSO method: Design 1 (left), Design 2 (middle), Design 3 (right).}\label{ISOiterations}
\end{figure}

\begin{figure}[h!]
\centering\includegraphics[width=1.0\linewidth]{Figures/Fig-iterPSO.pdf}
\caption{Convergence process of the PSO algorithm: Design 1 (left), Design 2 (middle), Design 3 (right).}\label{PSOiterations}
\end{figure}

Figure \ref{ShapeOpt} shows the 1000 optimal PEH designs (one for each event) marked with blue, yellow and red dots for Designs 1, 2 and 3, respectively. Additionally, the figure shows the isocurve of the natural frequencies for different geometries (red line) and optimal designs using harmonic excitations (grey area) identified in the benchmark problem (Case Study 1). The results show that for Design 1 and 2, the optimal geometries (blue and yellow dots) are aligned along the grey line, as expected. However, in Design 3, red dots show significant deviations from the grey line. These dispersion are explained by the discrepancies in predominant frequencies among the events as it is discussed next.

\begin{figure}[h!]
\centering\includegraphics[width=1.0\linewidth]{Figures/ShapeOpt.pdf}
\caption{Isocurves for fundamental frequencies $\omega_o$ (red lines). $(a)$ Optimal geometries for the 1000 Events in Design 1 (blue dots). $(b)$ Optimal geometries for the 1000 Events in Design 2 (yellow dots). $(c)$ Optimal geometries for the 1000 Events in Design 3 (red dots). The geometries related to events 2, 113, 304, 384, 781 and 718 are identified in three figures; also geometries for events 113 and 728 are denoted in the right figure. The geometries around the 2 Hz are marked by a rectangle in the left and central figures.}\label{ShapeOpt}
\end{figure}

To study the relationship between the dynamic characteristics of the device and the event frequency spectrum, Figure \ref{FRFevents} presents the comparison of FRFs of six optimal designs and the Fourier acceleration spectrum of their respective event for the three design scenarios. Six optimal designs are identified in Figure \ref{ShapeOpt} with the purpose to be compared, which correspond to events 2, 113, 304, 384, 781 and 718. First, note that the fundamental frequency of the piezoelectric devices is tuned with the predominant frequency of the acceleration spectrum. However, the acceleration peak is not always the one with the highest amplitude, such as the events 781 and 718 where the devices' fundamental frequency is tuned with the widest acceleration spectrum peak. Also, it is important to mention that there is consistency between the optimal FRFs for the three design scenarios since the fundamental frequencies coincide in the six studied events. 
\begin{figure}[h!]
\centering\includegraphics[width=1.0\linewidth]{Figures/FRFevents.pdf}
\caption{Comparison between the Fourier spectrum of the event acceleration signal and the FRFs of the optimal geometries obtained from the three design scenarios for events 2, 113, 304, 384, 781 and 718.}\label{FRFevents}
\end{figure}

Note that optimal designs within the grey line are those that generate the higher energy from their first vibration mode. This is valid for all PEHs in Designs 1 and 2. In this sense, there is consistency in these results, meaning that, by grouping the optimal designs around some key frequency, the corresponding events share same frequency characteristics. Figure \ref{FRFevents3} presents the Fourier spectra of the events associated with PEH design around the 2 Hz, which are identified by a rectangle in Figure \ref{ShapeOpt}-a and \ref{ShapeOpt}-b. As expected, it is seen that the predominated frequency is around 2 Hz, the same as the natural frequency of the optimal harvesters.
\begin{figure}[h!]
\centering\includegraphics[width=1.0\linewidth]{Figures/SpectrumEvents.pdf}
\caption{Comparison of the normalised Fourier spectra of event acceleration signal around 2 Hz in Designs 1 and 2.}\label{FRFevents3}
\end{figure}

To understand the higher dispersion of the optimal geometries for Design 3, Figure \ref{FRFevents2} presents the comparison between the FRFs of three optimal designs and the Fourier acceleration spectrum of their respective event. The three optimal designs are identified in Figure \ref{ShapeOpt}-c, which correspond to events 2, 131 and 725. The three devices have the first natural frequency of 2 Hz. The high dispersion is explained by analysing the second natural frequency of the FRF. The main difference between Designs 1 and 2, against Design 3 is in the second natural frequency, which is more sensitive to change in parameter $l$ rather than parameters $R$ or $H$. The change in parameter $l$ allows increasing the energy generation from the second mode of vibration, slightly decreasing the energy generation from the first one, leading to a higher energy overall. Therefore, the main conclusion from this study is that according to the spectral characteristics of an event, in some cases it is better to use devices that harvest energy only around the first natural frequency, while in others it is more efficient to harvest energy simultaneously from the first two natural frequencies. Despite the fact that it might reduce the energy generation in the first range in order to favour energy generation in the second. 
\begin{figure}[h]
\centering\includegraphics[width=1.0\linewidth]{Figures/FRF3dots.pdf}
\caption{Comparison between the Fourier spectrum of event acceleration signal and the FRFs of the optimal geometries (Design 3) from the three shape optimisation cases for events 2, 131 and 725.}\label{FRFevents2}
\end{figure}

The results of this section can be summarised as follows. The optimisation problem using the event acceleration response in the bridge yields the results, expected from the FRF analysis and parametric studies. Obtained results are consistent among the studied cases. It was found that not always the best option is to tune and maximise the energy generation in one frequency (prediction areas). Also, the natural frequency of the optimal device is not always close to the highest peak of the acceleration spectrum of the corresponding event. All these issues are considered by the direct optimisation of the events in the time domain, giving it greater robustness than the design obtained by simply tuning the natural frequency of the device with a target value. Nevertheless, the optimal designs from different events present a high dispersion in case 3, where one of the design parameters is the ratio between the PZT-layer length and the overall device length, which makes the design sensitive with respect to the second fundamental frequency. 

In practice, we are interested in designing one or a limited number of piezoelectric devices for a continuous generation; thus, it is not feasible to design a device for each event or perform an optimisation process in long time windows due to computational limitations. In that sense, the next section will present an optimisation framework for designing piezoelectric devices for a continuous generation based on the results presented in this section.


==> Sections/sectionX.tex <==
\section{Case Study: Optimisation of PEHs for an in-service Bridge using Time Series Excitation}
\label{S:X}

The cable-stayed bridge shown in Figure \ref{fig:fig1} and analysed in reference \cite{alamdari2019multi} is chosen as a case study in this work. The bridge has one traffic lane and one pedestrian lane with a maximum load capacity of 30 tons over the Great Western Highway in the state of New South Wales (NSW), Australia. The structural system consists of a composite steel-concrete deck spanning over 46.2m and an A-shaped steel pylon with a height of 33m. The width and the depth of the concrete deck are uniform at 6.30m and 0.16m, respectively. The deck is supported by four longitudinal girders which are internally attached by a set of seven cross girders (CGs), see Figure \ref{fig:sensor}. Sixteen semi-fan arranged pre-tensioned stayed-cables with a diameter of 38mm are anchored on a steel tower and cross girders.


\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\textwidth]{Figures/1.jpg}
\caption{Illustration of the cable-stayed bridge located in the state of NSW, Australia.}
	\label{fig:fig1}
\end{figure}

Although the bridge has only one traffic lane, the vehicles can travel in both directions because the traffic flow is not high. Also, the first natural frequencies are low, i.e., 2 and 3.5 Hz for the first two modes, respectively \cite{alamdari2019damage}.
Five parameters define the geometry of the harvester (as shown in Figure \ref{PEH-scheme}): the total length $L$, the aspect ratio $R = W/L$ (relation between the width $W$ and the total length $L$), dimensionless piezoelectric length $l = L_{pzt}/L$ (relation between the length of the piezoelectric layers $L_{pzt}$ and the total length $L$), the total thickness $h = h_{s} + 2h_p$, and the dimensionless piezoelectric thickness $H = h_p/h$ (relation between the thickness of a piezoelectric layer $h_p$ and the total thickness $h$). A bronze substructure and two PZT 5A piezoceramic sheets connected in series are considered. The corresponding material properties are given in Table \ref{mat_prop_demarqui22}.
First, a parametric study and optimisation study is carried out to understand how the piezoelectric device's design impacts the energy harvesting in the bridge when harmonic excitations are assumed. Remember that in previous works the design process remits to tuning the device with one of the resonance frequencies of the bridge, so this study serves as a benchmark problem to be compared with optimisation based on bridge's time series. A procedure to select the electrical resistance is presented. Second, an optimisation problem to maximise the energy harvesting from a bridge is formulated and solved. The optimal results are compared with the results from the optimisation assuming harmonic excitation. Finally, the optimisation procedure proposed in Section \ref{S:3} is formulated and solved. 

